StreamGS: Online Generalizable Gaussian Splatting Reconstruction for Unposed Image Streams

The advent of 3D Gaussian Splatting (3DGS) has advanced 3D scene reconstruction and novel view synthesis. With the growing interest of interactive applications that need immediate feedback, online 3DGS reconstruction in real-time is in high demand. However, none of existing methods yet meet the demand due to three main challenges: the absence of predetermined camera parameters, the need for generalizable 3DGS optimization, and the necessity of reducing redundancy. We propose StreamGS, an online generalizable 3DGS reconstruction method for unposed image streams, which progressively transform image streams to 3D Gaussian streams by predicting and aggregating per-frame Gaussians. Our method overcomes the limitation of the initial point reconstruction \cite{dust3r} in tackling out-of-domain (OOD) issues by introducing a content adaptive refinement. The refinement enhances cross-frame consistency by establishing reliable pixel correspondences between adjacent frames. Such correspondences further aid in merging redundant Gaussians through cross-frame feature aggregation. The density of Gaussians is thereby reduced, empowering online reconstruction by significantly lowering computational and memory costs. Extensive experiments on diverse datasets have demonstrated that StreamGS achieves quality on par with optimization-based approaches but does so 150 times faster, and exhibits superior generalizability in handling OOD scenes.

==> sec/_1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% The field of photo-realistic scene reconstruction and novel view synthesis from multi-view images has made significant progress due to the invention of neural 3D representations such as Neural Radiance Fields (NeRFs) \cite{mildenhall2021nerf}. However, the high computational cost for per-scene reconstruction through volume rendering and the reliance on known intrinsics and poses of input images limit its practical application. 

Recently, 3D Gaussian Splatting (3D-GS) has been proposed as a more efficient method for scene reconstruction and novel view synthesis. Utilizing rasterization-based rendering techniques \cite{zwicker2001ewa}, 3D-GS achieves fast reconstruction speeds and real-time rendering with high quality. Nevertheless, a time-consuming preprocessing step based on Structure from Motion (SfM) \cite{schonberger2016structure} is required before the training process to obtain the camera parameters of multi-view images and initialize the 3D Gaussians. Additionally, optimizing Gaussians by gradients of rendering loss still takes several minutes. Moreover, the optimization process is in a offline fashion since all the input images need to be gathered before the training, making it not applicable to online image streams of previously unseen scenes.  \ca{3DGS's inherent optimizatino is limited to extend to online}

Recently, generalizable 3D Gaussian Splatting has been investigated to accelerate scene reconstruction, with methods such as SplatterImage \cite{splatter-image}, pixelSplat \cite{pixelsplat}, and MVSplat \cite{mvsplat}. The main idea behind these studies is that each pixel can be represented as Gaussians, and the parameters of these pixel-aligned Gaussians can be directly decoded from the image using an image-to-image neural network \cite{splatter-image}. These methods typically employ a 2D encoder-decoder network to regress Gaussians by rendering loss, allowing the 3D-GS representation of the scene to be attained within a single feed-forward pass, enabling real-time scene reconstruction. However, existing generalizable 3D-GS methods are mostly monocular or binocular, supporting only sparse-view inputs. In multi-view cases, these feed-forward methods often regress the centers of Gaussians by stereo matching across views to reduce ambiguity, heavily relying on known poses and intrinsics. PixelSplat predicts pixel-wise probabilistic depth distributions for each view based on cross-view-aware epipolar features extracted by epipolar transformers \cite{he2020epipolar}, which takes camera parameters as inputs. MVSplat \cite{mvsplat} performs stereo matching based on cross-view features of each view to ensure that predicted Gaussians from different views are expressed in the same coordinate system, which also depends on accurate poses to build the cost volume \cite{costvolume}. Both pixelSplat \cite{pixelsplat} and MVSplat \cite{mvsplat} require all input images before the reconstruction to extract cross-view features and predict Gaussians through pose-dependent stereo matching, making it inaccessible to address online reconstruction of streams with numerous unposed images. Moreover, pixel-aligned prediction without Adaptive Density Control (ADC) process entails redundant Gaussians.
\ca{generalizable sparse-view methods, 1) requiring poses, 2) no aggregation.}

Scene reconstruction without known camera parameters has been extensively studied based on NeRFs, such as NoPo-NeRF \cite{bian2023nopenerf} and SC-NeRF \cite{scnerf}. Pose-free 3D Gaussian Splatting has also emerged as a significant topic due to the inefficiency of SfM preprocessing for pose estimation, with methods like CF-3DGS \cite{cfgs}. The key design of these approaches is to treat poses as learnable parameters and optimize them with 3D representations during reconstruction. CF-3DGS \cite{cfgs} initializes the pose of each incoming image based on depth priors and jointly optimizes them with 3D-GS, aiming to align the latest Gaussians with previously reconstructed scenes. However, optimization-based per-frame alignment significantly increases the time cost of reconstruction, making it impractical for handling image streams.
\ca{pose-free methods, not generalizable}

\begin{figure}
    \centering
    \includegraphics[width=1.1\linewidth]{figs/teaser2}
    \caption{Pipeline for Online Generalizable 3D Gaussian Splatting: The proposed method, StreamGS, processes image streams as input and predicts corresponding Gaussian streams to progressively reconstruct the entire scene.}
    \label{fig:teaser}
\end{figure}

Scene reconstruction from image streams has gained increasing attention due to its potential for interactive applications with real-time feedback to users \cite{surfelnerf, yan2024gsslam}. 
The online nature of streaming reconstruction differentiates it from common settings, posing additional challenges. (1) The full image set is inaccessible during reconstruction, preventing the use of SfM preprocessing to obtain camera parameters for each frame. 
(2) Moreover, offline reconstruction after gathering all frames is unsuitable for streaming reconstruction as it loses the advantage of providing intermediate feedback. (3) Additionally, per-frame alignment is a bottleneck to the efficiency of streaming reconstruction, significantly slowing down the process.
Existing generalizable feed-forward reconstruction networks and pose-free 3D-GS methods do not meet the requirements of streaming reconstruction. 
Per-frame optimization in pose-free 3D-GS methods \cite{cfgs} reduces efficiency, making it even slower than offline reconstruction.
Generalizable 3D-GS methods \cite{pixelsplat, mvsplat} only support two or three input views and heavily rely on known camera intrinsics and poses.

To address these challenges, we propose a generalizable pipeline for online 3D Gaussian Splatting dedicated to unposed image streams, named \textbf{StreamGS}. Given an unposed image stream, our goal is to progressively establish and continuously update the 3D-GS representation of the entire scene quickly in a feed-forward manner as new frames are received, as shown in Fig. \ref{fig:teaser}. 
% Existing generalizable feed-forward reconstruction networks and pose-free 3D-GS methods do not meet the requirements of streaming reconstruction. 
% Per-frame optimization in pose-free 3D-GS methods \cite{cfgs} reduces efficiency, making it even slower than offline reconstruction, while generalizable 3D-GS methods \cite{pixelsplat, mvsplat} only support two or three input views and heavily rely on known camera intrinsics and poses.
Our insight is that adjacent incoming frames provide sufficient correspondences for these sparse-view generalizable 3D-GS methods to predict consistent Gaussians within each frame. Our main design extends these binocular feed-forward networks to handle streaming input views without camera parameters. Inspired by MASt3R \cite{mast3r}, we directly predict Gaussians expressed in the same coordinate system instead of using stereo matching and estimate camera parameters from the predicted Gaussians. We extract correspondences among incoming frames and propose a feed-forward joint \textbf{adaptive refinement} based on these correspondences to enhance the consistency of Gaussians across views and align Gaussian predictions in the current frames with preceding reconstructions. 
Additionally, we utilize the extracted correspondences to prune redundant pixel-aligned Gaussians, thereby achieving \textbf{adaptive density control} of 3DGS. This approach allows StreamGS to predict Gaussians corresponding to the input image stream on-the-fly with only feed-forward passes.
Evaluated on large-scale datasets including Re10K \cite{re10k}, ACID \cite{acid}, MV-ImgNet \cite{mvimgnet}, DL3DV \cite{dl3dv}, and ScanNet \cite{scannet}, StreamGS achieves high novel synthesis quality comparable to the optimization-based method CF-3DGS \cite{cfgs} but with 150x faster reconstruction speed. Moreover, our method outperforms existing pose-dependent generalizable 3D-GS methods in evaluating out-of-domain scenes, demonstrating superior generalizability. 
In summary, our contribution is three-fold.
\begin{itemize} \item We propose a pipeline for online feed-forward reconstruction of streams with numerous images as inputs. \item We eliminate the need for pose annotations during the training and reconstruction of our generalizable model. \item We propose correspondence-based 3D-GS refinement and pruning modules to enhance consistency and reduce the memory cost of online reconstruction. \end{itemize}

\section{Related Works}
\paragraph{Generalizable 3D Gaussian Splatting.} Many recent studies aim to propose generalizable 3D-GS methods capable of predicting Gaussians within a single feed-forward pass. These works can be classified into two main categories: single-view reconstruction and multi-view reconstruction. Single-view reconstruction does not involve pose estimation as there are no multi-view constraints. Inspired by the insight from LRM \cite{lrm} that large transformer-based \cite{vaswani2017attention} backbone networks can learn 3D priors from large-scale 3D data, the potential of predicting Gaussians from a single image in a single feed-forward pass has been comprehensively explored. Numerous feed-forward models have been proposed, such as GRM \cite{grm}, TriplaneGS \cite{triplanegs}, and GMamba \cite{shen2024gamba}. However, these methods are primarily not applicable to multi-view scenarios as they always assume canonical poses.

Concurrently, many works focusing on multi-view inputs follow a similar paradigm, such as GS-LRM \cite{zhang2025gslrm}, LGM \cite{lgm}, and MVGMamba \cite{yi2024mvgamba}. They concatenate the input images with camera embeddings like Pl\"{u}cker rays to facilitate the network in learning the proper fusion of Gaussians from multi-view inputs. However, these large 3D backbone networks mostly perform well only on synthetic objects due to the shortage of large-scale scene-level 3D data in the real world. Referring to generalizable NeRF methods like pixelNeRF \cite{yu2021pixelnerf}, other research turns to multi-view stereo (MVS) matching to locate or initialize the centers of Gaussians, with other attributes decoded using a lightweight 2D encoder. Representative works with this design include MVSGaussian \cite{liu2025mvsgaussian}, pixelSplat \cite{pixelsplat}, and MVSplat \cite{mvsplat}. However, both camera ray embedding in large transformer-based models and stereo matching rely on known poses and intrinsics of each input view. Another main limitation of these methods is that they focus on sparse-view inputs. PixelSplat \cite{pixelsplat} and MVSplat \cite{mvsplat} only support up to three views. Therefore, existing generalizable 3D-GS models cannot address the problem of feed-forward reconstruction from endless image streams.

\paragraph{Pose-free 3D Gaussian Splatting.} Recently, many works have aimed to eliminate the need for Structure-from-Motion (SfM) preprocessing steps using COLMAP \cite{schonberger2016structure} software. Following the design of previous pose-free NeRF methods like NoPe-NeRF \cite{bian2023nopenerf}, Lu-NeRF \cite{lunerf}, and localRF \cite{localrf}, CF-3DGS \cite{cfgs} introduces depth priors into the optimization of 3D-GS and performs progressive reconstruction. As each new image arrives, CF-3DGS optimizes both the pose and 3D Gaussians of the input image based on its depths, aiming to align the 3D-GS from the new image with the preceding reconstruction. However, it still relies on known camera intrinsics. CF-3DGS is also not robust, as the accuracy of depth priors significantly impacts its reconstruction quality, limiting its application to common scenes. Moreover, it depends on thousands of optimization steps for each view, significantly extending the reconstruction time for each scene. Compared to generalizable 3D-GS models, current pose-free methods are so inefficient that they cannot be applied to image streams with a large number of frames.

\paragraph{Online 3D reconstruction of image streams.} Online 3D reconstruction has been extensively studied in the field of SLAM \cite{zhu2022nice, zhang2024improved, zou2022mononeuralfusion, zhu2024nicer, yan2024gsslam, yugay2023gaussianslam}. However, these methods typically involve additional information and most leverage SDF and NeRF as scene representations. NICE-SLAM \cite{zhu2022nice} uses RGB-D streams as input, with the reconstructed scene represented by NeRF. NICER-SLAM \cite{zhu2024nicer} relies on geometric priors, including surface normals and depths. SurfelNeRF \cite{surfelnerf} focuses on the novel view synthesis quality of online reconstruction with RGB streams, but it requires the poses and intrinsics of frames. Gaussian-SLAM \cite{yugay2023gaussianslam} reconstructs the scene using 3D-GS, but it also relies on RGB-D streams.

==> sec/_2_method.tex <==
\section{Methods}
\label{sec:method}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/pipeline.pdf}
    \caption{Overview}
    \label{fig:pipeline}
\end{figure*}

\paragraph{Overview.}
We propose a holistic pipeline of generative Gaussian splatting for online photo-realistic scene reconstruction. To reconstruct a scene, we begin with an image stream $\mathcal{I} = \left\{ \mathbf{I}^i\right\}_{i=1}^N$ consisting of $N$ unposed images. These images are divided into $T$ overlapping subsets using a sliding window of size $K$, which are sequentially processed over $T$ inference steps. 
At each inference step $t$, the objective is to estimate the Gaussian primitives $\mathcal{G}^t$ for the current image $\mathbf{I}_t$ by determining the conditional distribution of these Gaussian primitives, represented as $\mathcal{G}^t \sim \mathrm{Pr}\left(\mathbf{G}^t \mid \mathcal{G}^{0:t-1}\right)$.
% corresponding to the arriving subset of the sequence $\left\{ \mathbf{I}^k\right\}_{k=n_t}^{n_t+K}$ at step $t$. 
\todel{
 During each inference step $t$, our goal is to infer the conditional distribution of Gaussian primitives $\mathcal{G}^t \sim \mathrm{Pr}\left(\mathbf{G}^t \mid \mathcal{G}^{0:t-1}\right)$ corresponding to the arriving subset of the sequence $\left\{ \mathbf{I}^k\right\}_{k=n_t}^{n_t+K}$ at step $t$. 
 }
The complete set of Gaussian primitives representing the entire scene is constructed by concatenating the Gaussian primitives from all steps, $\mathcal{G} = \bigcup_{i=0}^{T-1} \mathcal{G}^t$.
\ca{mathcal or mathbf G?}
\begin{figure}[!htbp]
  \centering
  \begin{tikzpicture}
    \draw[thick] (0,0) rectangle (4,4);
    \node at (2,2) {Placeholder};
  \end{tikzpicture}
  \caption{Online reconstruction.}
  \label{fig:task}
\end{figure}

For simplicity, we only discuss the case between adjacent frames in the following statements. Note that our method do not rely on known extrinsics and intrinsics. In contrast, the input of group $i$ is sole two images denoted by $(\mathbf{I}^{t-1} \mid \mathbf{I}^t) \in \mathbb{R}^{H\times W\times 3} $. Our goal is to predict the Gaussian primitives $\mathbf{G}^i = \{ [\boldsymbol{\mu}^i_j, \alpha^i_j, \mathbf{\Sigma}^i_j, \mathbf{c}^i_j]\}_{j=1}^{N^i}$ in images, where $N^i$ is the number of primitives in the $i$-th image. Unlike pixelSplat \cite{pixelsplat} and MVSplat \cite{mvsplat}, $N^i$ is not always equal to $H \times W$ since we perform Feed-Forward Adaptive Density Control (ADC) to reduce number of primal pixel-aligned Gaussians efficiently.
\subsection{Joint Gaussians and Camera Motion Prediction}
\label{sec:gp}
\ca{better add the corresponding symbols or labels in fig:overview}
\paragraph{Geometry prediction.}
First, we need to reconstruct centers of Gaussian primitives within input frames. However, our inputs do not involve ground truth extrinsics and intrinsics of cameras, making the problem much more challenging. Based on poses of different views, previous generative Gaussian Splatting methods \cite{pixelsplat, mvsplat} always perform stereo matching across views to estimate depth maps per view, and then centers can be calculated from unprojection. Such manners can not be applied to pose-free cases. Instead, we employ DUSt3R \cite{dust3r} as a pixel-aligned 3D points predictor, serving as a rough prediction of Gaussians' centers. It directly outputs corresponding pointmaps, $\mathbf{X}^{t-1, t-1}$, $\mathbf{X}^{t, t-1} \in \mathbb{R}^{H \times W \times 3}$, of two input views, associated with confidence maps $\mathbf{C}^{t-1, t-1}$, $\mathbf{C}^{t, t-1} \in \mathbb{R}^{H \times W}$. The first element of superscripts represents the input images $\mathbf{I}^{t-1}$ and $\mathbf{I}^t$, and the second one indicates that both of them are expressed in the same camera coordinate frame of image $\mathbf{I}^{t-1}$. The confidence maps measure the certainty of pointmaps at each pixel, reflecting a prior-based estimation of reconstruction accuracy and difficulty. 

\ca{the definitions of pointmap, two view in the same camera coordnate are not easy to get, if others didn't know dust3r, some fig illustration?}

\ca{network design not discussed. 3D backbone? image encoder?}

\paragraph{Camera pose estimation.}
\ca{camera pose definition, P, intrinsics, extrincis...}
Given pointmap $\mathbf{X}^{t-1, t-1}$, the intrinsic parameters of image $\mathbf{I}^{t-1}$ can be estimated in a DUSt3R-like fashion:
\begin{equation}
\resizebox{.9\hsize}{!}{$ \hat{f}^{t-1} =  \arg \min\limits_{f^{t-1}} \Sigma_{i=0}^{W} \Sigma_{j=0}^{W} \parallel (i', j') - f^1 \dfrac{(\mathbf{X}^{t-1,t-1}_{i,j,0}, \mathbf{X}^{t-1,t-1}_{i,j,1})}{\mathbf{X}^{t-1,t-1}_{i,j,2}} \parallel, $}
\label{eq:focal}
\end{equation}
\ca{$f^1$??}
where $f^{t-1}$ is the focal length of the camera at $\mathbf{I}^{t-1}$, $(i',j')$ is the offset from the principle point, and $\mathbf{X}^{t-1,t-1}_{i,j,0}$ is the 0-$th$ coordinate value of pointmap $\mathbf{X}^{t-1,t-1}$ at pixel $(i,j)$. Intrinsic of $\mathbf{I}^2$ can be obtained following the same equation, based on pointmaps $(X^{t-1,t}, X^{t,t})$, \ca{mathbf} taking the reversed pair $(\mathbf{I}^t, \mathbf{I}^{t-1})$ as input. Moreover, we also can approximate relative pose $\mathbf{P}^{t} = [\mathbf{R}, \mathbf{t}]$ of $\mathbf{I}^{t}$ by solving the following points registration problem:
\begin{equation}
\resizebox{.9\hsize}{!}{$
\begin{aligned}
 [\hat{\mathbf{R}}^{t} \vert \hat{\mathbf{t}}^{t}] &= \arg \min\limits_{s, \mathbf{R}, \mathbf{t}} \sum_i^{H \times W} C_i^t \parallel s(\mathbf{R} \mathbf{X}_i^{t-1,t-1} + \mathbf{t}) - \mathbf{X}_{i}^{t-1,t} \parallel^2, \\
     &\, C_i^t = C_i^{t-1,t-1} C_i^{t-1,t}, 
\end{aligned}
$}
\label{eq:pts-reg}
\end{equation}
\ca{$C$?? mathbf}
where $s$ is a scale factor to adjust the focal of $\mathbf{I}^{t}$.


\paragraph{Cross-view registration refinement.}
\todel{
\paragraph{Centers alignment by match.} 
While the above estimation is efficient, the raw centers predicted by DUSt3R are not consistently aligned well with challenging cases like indoor scenes. Naturally, the accuracy of predicted centers of Gaussian primitives and poses of images is sensitive to noise of pointmaps. Moreover, we observed that in the settings of online reconstruction, the incoming frame are similar to neighboring frames since the camera motion of video is continuous. 
}
\ca{to revise. is the 3D backbone Dust3r? there's no camera output in figure 2 of 3D backbone. }
It inspires us to utilize the redundant matches between neighboring frames to refine the position of Gaussian centers and frame poses jointly. We employ the matching head of MASt3R \cite{mast3r} to extract local features $(\mathbf{f}^{t-1,t-1}, \mathbf{f}^{t,t-1}) \in \mathbb{R}^{H \times W \times d}$ of the input pair $(\mathbf{I}^{t-1}, \mathbf{I}^{t})$. 
Then, the correspondences between the two images can be derived from nearest reciprocal (NN) searching, satisfying the following condition:
\begin{equation}\label{eq:match}
\resizebox{.9\hsize}{!}{$
\begin{aligned}
 \mathcal{M}^{t-1,t} &= \{ i_k \leftrightarrow j_k \vert i_k = \mathrm{NN} (j_k) \ \mathrm{and}\ j_k = \mathrm{NN}(i_k) \}_{k=1}^{N}, \\
    & \mathrm{s.t.}\ \mathrm{NN}(i_k) = \underset{0 \leq j_k \leq H \times W}{\arg \min} \mid 1 - \cos <\mathbf{f}^{t-1}_{i_k}, \mathbf{f}^{t}_{j_k}> \mid,
\end{aligned}
$}
\end{equation}
\ca{inconsistent label: $\mathbf{f}^{t-1,t-1} $, $ \mathbf{f}^{t-1}$}
where $i_k, j_k$ are pixel index in image $\mathbf{I}^1, \mathbf{I}^2$ respectively, and the measurement of feature distance is cosine similarity. With $N$ correspondences found, a residual transform $\boldsymbol{\Delta} = [\Delta\mathbf{R}, \Delta\mathbf{t}]$ can be estimated following the same \cref{eq:pts-reg} during the coarse alignment, but only taking matched points into account. Then we apply the residual transform to the pointmap $\mathbf{X}^{t,t-1}$ to retain refined $\tilde{\mathbf{X}}^{t,t-1}$, and the pose of $\mathbf{I}^{t}$ is updated to $\tilde{\mathbf{P}}^{t}$ by performing PnP-RANSAC \cite{pnp, ransac} on 3D-2D correspondences derived from matches.
\ca{\mathbf{P} should be defined before, in camera pose estimation.}

% \paragraph{Features of other Gaussian parameters.} 
\paragraph{Gaussian parameter estimation.} 
Similar to other Feed-forward 3D-GS works \cite{mvsplat, pixelsplat, splatter-image}, we directly predict the feature of other Gaussian parameters at each pixel with a light-weight neural network $f_{\theta}$ as:
\begin{equation}
    \mathbf{f}_g^i = [\mathbf{q}^i, \boldsymbol{s}^i, \alpha^i, \mathbf{c}^i] = f_{\theta}([1/\mathbf{d}^i, \mathbf{I}^i]), i = \{t-1,t\},
\end{equation}
\ca{Duplicated notations: $\mathbf{f}$ already used as image feature, $\mathbf{R}$}

where $\mathbf{q}^i \in \mathbb{R}^{H \times W \times 4}$ and $\mathbf{s}^i \in \mathbb{R}^{H \times W \times 3}$ represent rotation quaternions and scales of pixel-aligned Gaussians at image $\mathbf{I}^i$. Then covariance matrix is built with $\boldsymbol{\Sigma}^i = \mathbf{R}(\mathbf{q}^i)\mathbf{s}\mathbf{s}^{\mathrm{T}} \mathbf{R}(\mathbf{q}^i)^\mathrm{T}$. The network takes depths $\mathbf{d}^i$ and images as inputs. \ca{which network? why use depth?} Depths can be obtained by transforming the coordinates system of pointmap from world space to camera space based on the refined intrinsic $\mathbf{K}^i$ and pose $\tilde{\mathbf{P}}^i$, which is formulated as $\mathbf{d}^i = \left( \mathbf{K}^{-1} (\tilde{\mathbf{P}}^i)^{-1} \tilde{\mathbf{X}}^{i,t-1} \right)_3 $. Note that $\mathbf{f}_g^i$ is not the final parameters since it needs to be merged first following Sec. \ref{sec:adc}.

\subsection{Feed-Forward ADC for Online Reconstruction}
\label{sec:adc}
With pixel-aligned Gaussian parameters $\mathbf{G}^i = [\boldsymbol{\mu}^i(\mathbf{X}^{i,1}), \mathbf{\Sigma}^i, \alpha^i, \mathbf{c}^i]$ of $N$ images, previous methods  \cite{pixelsplat, mvsplat, splatter-image, lgm} always naively take the concatenation of Gaussian primitives in each images as the final prediction, i.e., $\mathcal{G} = \bigcup_{i=1}^N \mathbf{G}^i$ and  $\vert \mathcal{G} \vert  = N \times H \times W$. However, this approach is both memory-intensive and inefficient in rendering, particularly when dealing with the continuous input of video frames during online reconstruction. Our key observation is that the Gaussian primitives in neighboring frames are excessive and prunable since they consistently share similar attributes in shape and color, and are closely distributed. A straightforward method for reducing these duplicated Gaussians from different views is to perform Gaussians down-sampling in 3D space \cite{instantsplat}. However, the down-sampling process necessitates traversing the 3D grid, resulting in a time complexity of $O(n^3)$, which does not meet the efficiency requirements for feed-forward reconstruction. It is noted that we have already acquired dense pixel-wise matches between neighboring frames from Eq. \ref{eq:match}. Therefore, we propose a novel feed-forward Adaptive Density Control  strategy based on revisiting these dense correspondences.
\ca{move some motivation-related content to intorduction.}

% \begin{figure}[!htbp]
%   \centering
%   \begin{tikzpicture}
%     \draw[thick] (0,0) rectangle (4,4);
%     \node at (2,2) {Placeholder};
%   \end{tikzpicture}
%   \caption{Merging process}
%   \label{fig:task}
% \end{figure}

\paragraph{Feature wrapping by matches.} The primary advantage of 2D correspondences is that they are able to convert the computationally intensive 3D Gaussian merge process into a more efficient 2D pixel-wise one. This significantly enhances computational efficiency. Initially, the feature of Gaussian parameters $\mathbf{f}_g^{t}$ of the frame $\mathbf{I}^i$ can be aligned to the previous frame $\mathbf{I}^{t-1}$ using the following wrapping:
\begin{equation}
    \mathbf{f}_g^{t,t-1}(j) = \begin{cases} 
        \mathbf{f}_g^{t}(k) & \text{if } (j, k) \in \overline{\mathcal{M}}^{t-1,t} \\
        \mathbf{f}_g^{t-1}(j) & \text{else,} \\
        \end{cases}
\end{equation}
\ca{use $\mathbf{g}$ instead?}
where $\mathbf{f}_g^{t,t-1}$ is the feature of Gaussian primitives in the frame $\mathbf{I}^{t}$ aligned to $\mathbf{I}^{t-1}$. Instead of using the raw correspondences set $\mathcal{M}^{t-1,t}$ in Eq. \ref{eq:match}, we use the extended set $\overline{\mathcal{M}}^{t-1,t}$, which includes matches of neighboring pixels such as $(i+1, j+1)$ in addition to the initial $(i,j)$. It serves as a type of anti-aliasing technique to reduce void pixels within the wrapped feature map. As for the unmatched pixels, we simply replicate the corresponding feature vector within $\mathbf{f}_g^{t-1}$. With the aligned feature, the Gaussian feature of two frames can be merged with a light-weight neural network, which is defined as:
\begin{equation}
    \hat{\mathbf{f}}_{g^M}^{t-1, t} = [\hat{\mathbf{q}}^{t}, \hat{\boldsymbol{s}}^{t}, \hat{\alpha}^{t}, \hat{\mathbf{c}}^{t}] = g_{\phi}([\mathbf{f}_{g}^{t,t-1}, \mathbf{f}_g^{t-1}, \mathbf{f}^{t}, \mathbf{f}^{t-1}]),
\end{equation}
where we concatenate the matching features $\mathbf{f}^{t}$ and $\mathbf{f}^{t-1}$ (\cref{eq:match}) to facilitate the learning of the merge. In this way, every matched pair of Gaussian primitives between $\mathbf{I}^{t}$ and $\mathbf{I}^{t-1}$ is aggregated into a single one, reducing the number of Gaussians by $N^i$. Without gradient back-propagation of rendering loss in the original 3D-GS \cite{3dgs}, our ADC process runs exceptional fast. In terms of the input group, the final prediction of Gaussian primitives $\mathcal{G}^{t}$ consists of the merged Gaussians and the unmatched Gaussians at each frame.


\subsection{Video reconstruction.} For online reconstruction of a video sequence with multiple input groups, we perform group-wise alignment following the same steps as described above. After alignment, the Gaussian primitives at each frame $\mathcal{G}^t$ are expressed in the same coordinate system, and the prediction of the video is progressively updated by $\mathcal{G} = \bigcup_{i=0}^{T-1} \mathcal{G}^t$.
\subsection{Optimization}
\label{sec:opt}
The optimization of the Gaussian parameters encoder network, $f_{\theta}$, and the merge network, $g_{\phi}$, involves both a rendering loss function and a reconstruction loss function:
\begin{equation}
\resizebox{.9\hsize}{!}{$
    \begin{aligned} \mathcal{L}(\mathbf{I}^i, \hat{\mathbf{I}}^i, \hat{\mathbf{I}}^i_M) &= \mathcal{L}_{\mathrm{render}}(\mathbf{I}^i, \hat{\mathbf{I}}^i) + \mathcal{L}_{\mathrm{recon}}(\hat{\mathbf{I}}^i, \hat{\mathbf{I}}^i_M) \\ &= \parallel \mathbf{I}^i - \hat{\mathbf{I}}^i \parallel_2 + \parallel \mathbf{I}^i - \hat{\mathbf{I}}^i \parallel_{\mathrm{LPIPS}} + \parallel \hat{\mathbf{I}}_{\mathrm{M}}^i - \hat{\mathbf{I}}^i \parallel_2, \end{aligned},
    $}
\end{equation}
where  $\mathbf{I}^i$ is the ground truth frame, $\hat{\mathbf{I}}^i$ is the rendered image with full Gaussian primitives before the merge process, and $\hat{\mathbf{I}}_{\mathrm{M}}^i$ is the rendered image with merged Gaussians. Due to the lightweight nature of the two networks, the algorithm converges quickly within thousands of steps. The reconstruction loss term facilitates the merge network in fusing the pixel-aligned Gaussian parameters from different frames, aiming to render the same frame as before the merge process but with significantly fewer Gaussian primitives.
